Visual Transformer for Task-aware Active Learning

Pool-based sampling in active learning (AL) represents a key framework for an-notating informative data when dealing with deep learning models. In this paper, we present a novel pipeline for pool-based Active Learning. Unlike most previous works, our method exploits accessible unlabelled examples during training to estimate their co-relation with the labelled examples. Another contribution of this paper is to adapt Visual Transformer as a sampler in the AL pipeline. Visual Transformer models non-local visual concept dependency between labelled and unlabelled examples, which is crucial to identifying the influencing unlabelled examples. Also, compared to existing methods where the learner and the sampler are trained in a multi-stage manner, we propose to train them in a task-aware jointly manner which enables transforming the latent space into two separate tasks: one that classifies the labelled examples; the other that distinguishes the labelling direction. We evaluated our work on four different challenging benchmarks of classification and detection tasks viz. CIFAR10, CIFAR100,FashionMNIST, RaFD, and Pascal VOC 2007. Our extensive empirical and qualitative evaluations demonstrate the superiority of our method compared to the existing methods. Code available: https://github.com/razvancaramalau/Visual-Transformer-for-Task-aware-Active-Learning

==> sections/raz_method.tex <==
\section{Method}
\begin{figure*}
    \centering
    \includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=1.0\textwidth]{figures/pipeline2.pdf}
    \caption{This diagram depicts the proposed pipeline. We pass both the labelled and unlabelled examples through the same CNN and extract the visual features of each images encoded in the form of $C$ number of channels.
    These channels are turned into \emph{Visual Tokens} and feed into the Transformer. The output of the 
    Transformer are feed into the bifurcated branches to minimize both the learner's objective  
    class cross entropy loss from the labelled examples and the sampler's objective  binary cross entropy to minimize labelled vs unlabelled from both the labelled and unlabelled examples.}
    \label{fig:pipeline}
\end{figure*}

% \textcolor{red}{ Things to mention/ add in justifications:
% \begin{itemize}
%     \item Hard parameter sharing - most common practice that shares the back-end layers to the task-specific outputs.
%     \item We alternate the gradient back-propagation between the sampler and the task branch with every batch. This adds an inductive bias while avoiding both over-fitting the data and the random noise. 
%     \item Joint learning offers a higher degree of generalisation by improving the feature representations. In a limited budget application, there is the risk of over-fitting. However, this can be overcome with the addition of more unlabelled images. Our joint learning proposal benefits of this advantage.
%     \item Another attribute of the pipeline consists in the preservation of the most meaningful features during the learning stage. Therefore, we focus the selection of the sampler to the most uncertain samples. In this manner, we can fully exploit the entire data representation within a few query steps.
% \end{itemize}
% }

In this Section, we start with the formal definition of the pool-based Active Learning in general followed by our contributions. 

% \subsection{Pool-based Active Learning}
% \label{sec3.1}
\noindent \textbf{Pool-based Active Learning:}
% \label{sec3.1}
% Broadly, active learning can be represented by three main components: learner, sampler and oracle or annotation system. The learner is responsible with training and performing the downstream task, while the sampler selects the new informative data for improving the system. Moreover, the sampler can also guide the oracle, responsible with the annotation process, in expanding to uniform datasets. Specifically, we consider deep CNNs as learners given the recent success in vision tasks \cite{he2016deep, Simonyan2015VeryRecognition}. However, due to their high number of parameters and converging complexity, the active learning framework can be deployed only under a pool-based scenario \cite{settles.tr09}.
%
% Given a large pool of unlabelled data $\mathbf{x_U} \in \mathbf{U}_{pool}$, we apply a cold-start to our learning model by randomly selecting and labelling an initial set $\mathbf{x_L}_0, \mathbf{y_L}_0 \in \mathbf{L}_{0} \subset \mathbf{U}_{pool}$. We define a budget $b$ to sample unlabelled examples over multiple selection stages. After each stage, the new batch $\mathbf{x_L}_1, \mathbf{y_L}_1 \in \mathbf{L}_1$ is annotated and plugged for re-training the learner.
%
% Finally, the main objective of the pool-based AL scenario is to obtain fast generalisation of the learner with the least number of labelled subsets $\mathbf{L}_n$. Therefore, our contribution lies on optimizing the learner with the most informative samples while bringing down the annotation cost.
Given a large pool of unlabelled data $\mathbf{x_U} \in \mathbf{U}_{pool}$, the pipeline begins with a cold-start training of the model by randomly selecting a 
small subset and labelling an initial set $\mathbf{x_L}_0, \mathbf{y_L}_0 \in \mathbf{L}_{0} \subset \mathbf{U}_{pool}$. The performance of the initial model
is crucial for the end outcome of the the framework~\cite{csal} for model-based active learning. Our contribution lies in addressing this problem which is 
also commonly known as \emph{cold-start} problem. If $b$ is the budget to sample unlabelled examples over multiple selection stages, 
the main objective of the pool-based AL scenario is to obtain fast generalisation of the learner with the least number of labelled 
subsets $n$ in order to set the budget minimum. $\forall i \in n $,  $L_i = (\mathbf{x_L}_i, \mathbf{y_L}_i) \subset \mathbf{U}_{pool}$  
represents the annotated examples in every $\i^{th}$ batch.

% Finally, the main objective of the pool-based AL scenario is to obtain fast generalisation of the learner with the least number of labelled subsets $\mathbf{L}_n$. Therefore, our contribution lies on optimizing the learner with the most informative samples while bringing down the annotation cost.



\subsection{Visual Transformer in Joint Active Learning}

Under the pool-based scenario, we propose an AL framework that combines the sampler with the learner in an end-to-end task-aware training scheme. Thus, first we add a labelled vs unlabelled discriminator to the learner's objective for selecting samples later on. Then, we modularly integrate a Visual Transformer as a bottleneck for the learner. Finally, we train the joint-learning loss that minimizes both learner and discriminator objective functions. During the selection stage, we select the most uncertain unlabelled examples when passing them through the discriminator branch. The pipeline is visually depicted for the image classification task in Figure \ref{fig:pipeline}.  Furthermore, we detail and motivate our proposal in the next sections.

\subsubsection{Joint Active Learning}
The AL framework is composed of two parts: the task-aware learner-sampler training and the visual transformer integration. Here, we present the former.

Following the setup from section \ref{sec3.1}, the initial labelled set is $\mathbf{x_L}_0, \mathbf{y_L}_0 \in \mathbf{L}_{0}$. For most vision applications, the backbone of the learner is a feature extractor commonly formed of CNNs. We consider the output of this block as $f(\mathbf{x_L}_0 ; \theta)$, where $\theta$ are the parameters of these layers. Consequently, the objective function is targeted with a feed-forward network for the downstream task. In the experiment section, we approach both image classification and object detection tasks. The loss for the former is cross-entropy $\mathcal{L}_{CE}(\mathbf{x_L}_0, \mathbf{y_L}_0; \theta)$, whilst for detection is the combination of confidence and localisation loss $\mathcal{L}_{SSD}(\mathbf{x_L}_0, \mathbf{y_L}_0; \theta)$ \cite{ssd}.

Given the image classification task, we propose to add a separate output branch from the feature extractor that is acting as sampler in the selection stage. During training, this branch consists of a discriminator that distinguishes labelled samples from the unlabelled. Therefore, both $(\mathbf{x_L}_0, \mathbf{y_L}_0)$ and $(\mathbf{x_U}_0 \in \mathbf{U}_{0} \subset \mathbf{U}_{pool})$, a subset from the unlabelled pool, are used when training the learner. However, only the label vs unlabelled discriminator back-propagates a binary cross-entropy loss, $\mathcal{L}_{BCE}$, when unlabelled are inferred. This hard-parameter sharing is common practice in multi-tasking where the back-end layers are shared.

Moreover, we alternate the gradient back-propagation between the sampler and the task branch with every batch. This adds an inductive bias while avoiding over-fitting the data or the random noise. While training in an end-to-end fashion, the joint learning loss for image classification when passing labelled data can be defined as:

\begin{equation}
    \mathcal{L}_{JL} = \lambda_1 \mathcal{L}_{CE}(\mathbf{x_L}_0, \mathbf{y_L}_0; \theta_1) + \lambda_2 \mathcal{L}_{BCE}(\mathbf{x_L}_0, 1 ; \theta_2),
    \label{eq:1}
\end{equation}
where $\lambda_1, \lambda_2$ are the weighting factors corresponding to each task. When we infer $(\mathbf{x_U}_0, 0)$, the downstream task is turned off, thus, $\lambda_1$ is 0. 
From a design perspective, the discriminator branch stacks two feed-forward layers activated with a sigmoid binary output.

Recently, the state-of-the-art for deep active learning has been gained by model-based methods like Learning Loss\cite{Yoo2019LearningLearning}, VAAL\cite{Sinha2019VariationalLearning}, CDAL\cite{cdal} and UncertainGCN\cite{ugcn}. These fundamentally comprise of dedicated trainable models to sample unlabelled data. Apart from Learning Loss, the downfall of these methods is the sub-optimal multi-stage training processes. Also, in limited budget scenarios, the risk of over-fitting appears from the initial cold-start sampling.

Our approach overcomes these limitations by offering a higher degree of generalisation while improving the feature representation with the addition of unlabelled data. Furthermore, the pipeline preserves the most meaningful spatial features during the learning stage.


\subsubsection{Visual Transformer Bottleneck}

Before delving in the selection process, we analyse the key module of this proposal, the \emph{visual transformer bottleneck}. Therefore, we incorporate this block initially to boost the performance of the learner. Secondly, while training, we back-propagate both labelled and unlabelled images to distinguish their inner feature relationship with the discriminator. In this manner, the transformer enriches the learner in an unsupervised way with the higher order of representations. This module has been successfully deployed recently to many applications as it retains better the long-range dependencies. 

In \cite{vi}, patches of the image are considered input tokens to the transformer for classification task. However, a more recent analysis \cite{vt} compressed the features of CNN backbones to visual tokens while the transformer acted as the final convolutional layer. Inspired from these works, we integrate a visual transformer as a bottleneck between the feature extractor and the split of the two tasks (the sampler and the main objective). Thus, the inputs to the transformer are batches of feature maps on multiple channels $f(\mathbf{x}; \theta) \in \mathbb{R}^{B \times HW \times C}$.

Differently from \cite{vi, vt}, we want our AL framework to be least intrusive to the learner's architecture. This will allow the methodology to be plugged to various designs and applications. We therefore preserve the features from the CNN by not reducing them to visual tokens. Similarly to GCNs \cite{kipf2016semi}, we want to explore the relationships between the nodes of the graph. However, given our input $f(\mathbf{x}; \theta)$, we propose to deploy the transformer blocks within the batch $B$. Consequently, all the channels of the feature maps from each batch are considered as tokens. Although, in the standard architecture \cite{attall}, the inputs to the transformer are positional encoded, this does not apply in our scenario where the order of the images is irrelevant. To simplify furthermore the transformer's architecture, we exclude the decoder part as another domain is not required.

Defined in \cite{attall}, the main building blocks of the transformers' encoder are a batch self-attention block and a point-wise feed-forward network with residuals and layer normalisation. For the self-attention, we transpose to the batch and concatenate the feature maps so that $f_T(\mathbf{x}; \theta) \in \mathbb{R}^{HWC \times B}$. The key, query and value matrices ($\mathbf{W}_{\mathbf{K}_{att}}, \mathbf{W}_{\mathbf{Q}_{att}}, \mathbf{W}_{\mathbf{V}_{att}}$) are packed together to model the interactions between the features. This also favors inner-domain relationships as batch normalisation is commonly used in CNNs as regularisation. The operations of the batch self-attention are summarised as follows:

\begin{equation}
    \mathbf{T}_{att} = f_T(\mathbf{x}; \theta) + \frac{\textrm{softmax}((f_T(\mathbf{x}; \theta)\mathbf{W}_{\mathbf{K}_{att}})(f_T(\mathbf{x}; \theta)\mathbf{W}_{\mathbf{Q}_{att}})^T)}{\sqrt{dim_{\mathbf{K}_{att}}}}(f_T(\mathbf{x}; \theta)\mathbf{W}_{\mathbf{V}_{att}}),
    \label{eq:2}
\end{equation}

where $\mathbf{T}_{att}$ and $\textrm{softmax}$ are the output of the batch self-attention layer its activation function. While keeping the dynamics within the batch, we pass $\mathbf{T}_{att}$ through the point-wise feed-forward network. We define $\mathbf{T}_{out}$ the output of this block. The following equation underlines its processes:

\begin{equation}
    \mathbf{T}_{out} = \mathbf{T}_{att} + \sigma(\mathbf{T}_{att}\mathbf{W}_{f_1})\mathbf{W}_{f_2},
    \label{eq:3}
\end{equation}

where $\mathbf{W}_{f}$ are the weights from the feed-forward network and $\sigma$ represents the sigmoid activation function.

In \cite{vt}, it has been shown that the self-attention aggregation function retains better the diverse concepts than the GCN. Despite this, we conduct further analysis in the AL framework in the experiment section. With the aforementioned implementation of our proposal, we move to the final process which consists in the selection of the unlabelled data.

% The CNNs are designed to extract local spatial information from images. Thus, they lack of non-local relationships from far patches.

\subsection{Sampling the unlabelled data}

To review, the proposed AL framework trains jointly both learner and sampler. As a bottleneck, a visual transformer is added between the feature extractor and the two task branches. Combining the unlabelled and labelled data helps in preserving the most meaningful features during the learning stage. Moreover, the transformer will be exposed also to the unlabelled data dependencies. This happens as the task of the sampler is to classify the labelled from the unlabelled. The two are categorised as 1 or 0, respectively. If the unlabelled examples $\mathbf{x_U}_0 \in \mathbf{U}_{0}$ are easily differentiated by the sampler, we want to target for selection the most uncertain $\mathbf{x_U} \in \mathbf{U}_{pool}$.

Similarly, it has been done in an adversarial manner by VAAL \cite{Sinha2019VariationalLearning}, although their AL framework is not linked with the main task. Therefore, we derive our selection principle from UncertainGCN\cite{ugcn}. Given a budget of $b$ points, we infer entire unlabelled pool and select the samples with the lowest posterior probability of the discriminator branch. We notate $P_S$ as the confidence score of the posterior. Considering the first selection stage, we can evaluate the new labelled set $\mathbf{L}_1$ with:

\begin{equation} \label{eq:3}
    \mathbf{L}_1 = \mathbf{L}_0  \cup \argmax_{i=1\cdots b} P_S( \mathbf{x_U}; \theta_2).
\end{equation}

We compute the  $\argmax$ because the highest confidence score for the unlabelled is when $P_S( \mathbf{x_U}; \theta_2)$ is closer to 0. This selection process along with re-training is repeated until the targeted performance of the downstream task is reached.

For convenience, we denote the proposed AL framework as \emph{TJLS}( Transformer with Joint Learning Sampler). In the next part, we thoroughly quantify the stated method and motivations. Furthermore, to observe the impact of the transformer bottleneck, we also investigate the pipeline \emph{JLS} without it.  

% \subsubsection{Visual Transformer Learner}
% Before delving in the selection process, we analyse the key module of this proposal, the \emph{visual transformer bottleneck}. Therefore, we incorporate this block initially to boost the performance of the learner. Secondly, while training we back-propagate both labelled and unlabelled images to distinguish their inner feature relationship with the discriminator. In this manner, the transformer enriches in an unsupervised way these representations while creating two sub-domains: one for the main task, another for data annotation. 

% Given a deep CNN network, the front-end part is commonly a feature extractor that encodes distributed spatial information of the input images. The outputs of the feature extractor are batches of feature maps split on multiple channels $\mathbf{F} \in \mathbb{R}^{HW \times C}$. Following \cite{vi,vt}, a pre-processing step condenses the feature maps to a few words referred as \emph{visual tokens}. Thus, we apply a point-wise convolution by packing the queries and keys in $S$ semantic groups as $\mathbf{W}_{QK} \in \mathbb{R}^{C \times S}$. Then, pixel-level self-attention is obtained from softmax activations when combined again with input $\mathbf{F}$. Furthermore,
% to maximize the values of the semantic representations between the channels, we multiply $\mathbf{F}$ with $\mathbf{W}_{V} \in \mathbb{R}^{C \times C'}$. Finally, the self-attention maps are encapsulated under the new $C'$ channels. The \emph{visual tokens} $\mathbf{T} \in \mathbb{R}^{S \times C'}$ can be outlined under:
% \begin{equation}
%     \mathbf{T} = \textrm{softmax}(\mathbf{F}\mathbf{W}_{\mathbf{QK}})^T\mathbf{F} (\mathbf{F}\mathbf{W}_\mathbf{V}).
%     \label{eq:1}
% \end{equation}
% Similarly to NLP tasks, we also want to keep the sense of order between our tokens by learning the positional embedding. This way we assure controlled sparsity of the high-order information.

% Although the obtained visual tokens comprise the spatial self-attention under the weighted channels $C'$, we still have to model the interactions between them. To address this, we choose the transformer architecture \cite{attall}. When compared with GCNs \cite{kipf2016semi}, it was shown to better model the high-order relationships between features. Moreover, this is handled within a few tokens in contrast to a large number of graph nodes. However, we simplify the transformer architecture only to the encoder as there is no need in decoding to new tokens. Defined in \cite{attall}, the two stages of the encoder are a self-attention and a point-wise fully-connected network with residuals and layer normalisation. These operations are applied to the visual tokens as follows:
% \begin{equation}
%     \mathbf{T}_{att} = \mathbf{T} + \frac{\textrm{softmax}((\mathbf{T}\mathbf{W}_{\mathbf{K}_{att}})(\mathbf{T}\mathbf{W}_{\mathbf{Q}_{att}})^T)}{\sqrt{dim_{\mathbf{K}_{att}}}}(\mathbf{T}\mathbf{W}_{\mathbf{V}_{att}}),
%     \label{eq:2}
% \end{equation}

% \begin{equation}
%     \mathbf{T}_{out} = \mathbf{T}_{att} + \sigma(\mathbf{T}_{att}\mathbf{W}_{f. _1})\mathbf{W}_{f_2}.
%     \label{eq:3}
% \end{equation}
% where $\mathbf{T}_{att}, \mathbf{T}_{out} \in \mathbb{R}^{S \times C'}, \mathbf{W}_{att}, \mathbf{W}_{f}$ are the output tokens and weights from the self-attention and the fully-connected network, respectively; $\sigma$ represents the sigmoid activation function.

% To finalize the transformer, because of transferring the visual tokens to two tasks, corresponding to learner and sampler, we employ a multi-head attention design. This permits in handling the two sub-domains with visual tokens dedicated for both objective functions.
% \subsubsection{End-to-end Sampler training}

% The second part of our proposal consists of adding a labelled vs unlabelled discriminator as a separate output after the visual transformer. While  labelled samples are propagated to the downstream task branch during training the learner, we also infer together the unlabelled samples to the discriminator. Therefore we train the learner end-to-end in a multi-task optimisation. Once the training is finished, we pass again only the unlabelled examples to the learner for selection. Finally, the sampler will query the most uncertain unlabelled data.

% The main reason of this module integration lies in enriching the learner's feature domain with unlabelled images while they are inherited in the visual transformer.
% Secondly, by training our sampler with the learner we reduce considerably the sampling time similarly to Learning Loss \cite{Yoo2019LearningLearning}. However, when back-propagating the discriminator loss, the feature extractor and the transformer expands its spatial and long-range dependencies.

% Our discriminator is composed of two fully-connected layers optimizing a binary cross-entropy loss. 
